The Fourier Evaluation of Tracings and Acidosis in Labor: the FETAL Technique

Adequate fetal and neonatal development depend upon the presence of a normal acid-base environment during pregnancy and the smooth transition from intra-uterine to extra-uterine life. Current methods to assess fetal pH and acid-base status are invasive and carry significant maternal and fetal risks. Given these limitations, obstetrical care providers developed the electronic fetal monitoring (EFM) system, a non-invasive tool, which evaluates beat-to-beat fetal heart rate (FHR) patterns in order to predict fetal oxygenation status in real-time. Every year, about 85 percent of the approximately 4 million live births in the United States are evaluated using EFM. Unfortunately, though there is ample physiological evidence that FHR patterns are inextricably linked to fetal acid-base status, the use of EFM has not been shown to reliably predict neonatal pH, nor has it reduced the incidence of adverse perinatal outcomes, including long-term neurological morbidity and cerebral palsy (CP). The poor specificity associated with the current interpretation of the EFM therefore leads to a paradox we have henceforth defined as the Obstetrical Paradox. In this study, we develop and seek to determine whether a novel, non-invasive method known as the FETAL technique (Fourier Evaluation of Tracings and Acidosis in Labor), which applies the Fourier Transform to EFM tracings and determines the spectral frequency distributions of the FHR, improves the assessment of the fetal pH in real time. We hypothesize that the improvement in the sensitivity and specificity of the EFM with the use of the FETAL technique will lead to a significant reduction in the rate of neonatal hypoxic injury and in the rate of caesarean deliveries for suspected fetal distress. The implications of a successful application of the FETAL technique would have paradigm-shifting consequences in the provision of modern obstetrical care.

==> references.tex <==
@article{parer2006fetal,
  title={Fetal acidemia and electronic fetal heart rate patterns: Is there evidence of an association?},
  author={Parer, JT and King, T and Flanders, S and Fox, M and Kilpatrick, SJ},
  journal={The Journal of Maternal-Fetal \& Neonatal Medicine},
  volume={19},
  number={5},
  pages={289--294},
  year={2006},
  publisher={Taylor \& Francis}
}

@article{alfirevic2017continuous,
  title={Continuous cardiotocography (CTG) as a form of electronic fetal monitoring (EFM) for fetal assessment during labour},
  author={Alfirevic, Zarko and Gyte, Gillian ML and Cuthbert, Anna and Devane, Declan},
  journal={Cochrane database of systematic reviews},
  number={2},
  year={2017},
  publisher={John Wiley \& Sons, Ltd}
}

 @article{low1981prediction,
  title={The prediction of intrapartum fetal metabolic acidosis by fetal heart rate monitoring},
  author={Low, JA and Cox, MJ and Karchmar, EJ and McGrath, MJ and Pancham, SR and Piercy, WN},
  journal={American Journal of Obstetrics and Gynecology},
  volume={139},
  number={3},
  pages={299--305},
  year={1981},
  publisher={Elsevier}
}

@article{ray2017intrapartum,
  title={Intrapartum cardiotocography and its correlation with umbilical cord blood pH in term pregnancies: a prospective study},
  author={Ray, Chandrima and Ray, Alokananda},
  journal={Int J Reprod Contracept Obstet Gynecol},
  volume={6},
  number={7},
  pages={2745--52},
  year={2017}
}

@article{low1999predictive,
  title={Predictive value of electronic fetal monitoring for intrapartum fetal asphyxia with metabolic acidosis},
  author={Low, James A and Victory, Rahi and Derrick, E Jane},
  journal={Obstetrics \& Gynecology},
  volume={93},
  number={2},
  pages={285--291},
  year={1999},
  publisher={Elsevier}
}

@article{campanile2018intrapartum,
  title={Intrapartum cardiotocography with and without computer analysis: a systematic review and meta-analysis of randomized controlled trials},
  author={Campanile, Marta and D’Alessandro, Pietro and Della Corte, Luigi and Saccone, Gabriele and Tagliaferri, Salvatore and Arduino, Bruno and Esposito, Giuseppina and Esposito, Francesca Giovanna and Raffone, Antonio and Signorini, Maria Gabriella and others},
  journal={The Journal of Maternal-Fetal \& Neonatal Medicine},
  pages={1--7},
  year={2018},
  publisher={Taylor \& Francis}
}

@article{talari2017advances,
  title={Advances in Fourier transform infrared (FTIR) spectroscopy of biological tissues},
  author={Talari, Abdullah Chandra Sekhar and Martinez, Marcela A Garcia and Movasaghi, Zanyar and Rehman, Shazza and Rehman, Ihtesham Ur},
  journal={Applied Spectroscopy Reviews},
  volume={52},
  number={5},
  pages={456--506},
  year={2017},
  publisher={Taylor \& Francis}
}

@article{pumprla2002functional,
  title={Functional assessment of heart rate variability: physiological basis and practical applications},
  author={Pumprla, Jiri and Howorka, Kinga and Groves, David and Chester, Michael and Nolan, James},
  journal={International journal of cardiology},
  volume={84},
  number={1},
  pages={1--14},
  year={2002},
  publisher={Elsevier}
}

@article{akselrod1981power,
  title={Power spectrum analysis of heart rate fluctuation: a quantitative probe of beat-to-beat cardiovascular control},
  author={Akselrod, Solange and Gordon, David and Ubel, F Andrew and Shannon, Daniel C and Berger, AC and Cohen, Richard J},
  journal={science},
  volume={213},
  number={4504},
  pages={220--222},
  year={1981},
  publisher={American Association for the Advancement of Science}
}
